Scalable High-Performance Fluxonium Quantum Processor

The technological development of hardware heading toward universal fault-tolerant quantum computation requires a large-scale processing unit with high performance. While fluxonium qubits are promising with high coherence and large anharmonicity, their scalability has not been systematically explored. In this work, we propose a superconducting quantum information processor based on compact high-coherence fluxoniums with suppressed crosstalk, reduced design complexity, improved operational efficiency, high-fidelity gates, and resistance to parameter fluctuations. In this architecture, the qubits are readout dispersively using individual resonators connected to a common bus and manipulated via combined on-chip RF and DC control lines, both of which can be designed to have low crosstalk. A multi-path coupling approach enables exchange interactions between the high-coherence computational states and at the same time suppresses the spurious static ZZ rate, leading to fast and high-fidelity entangling gates. We numerically investigate the cross resonance controlled-NOT and the differential AC-Stark controlled-Z operations, revealing low gate error for qubit-qubit detuning bandwidth of up to 1 GHz. Our study on frequency crowding indicates high fabrication yield for quantum processors consisting of over thousands of qubits. In addition, we estimate low resource overhead to suppress logical error rate using the XZZX surface code. These results promise a scalable quantum architecture with high performance for the pursuit of universal quantum computation.

==> sections/8_old_QEC.tex <==
\section{\label{sec:qec}Toward logical qubits}
%Introduce quantum error correction. What is the general idea? Introduce stabilizer code. 
While the gate errors we simulate is low, with the best two-qubit gate fidelity in the range of $10^{-6}$ in the absence of decoherence (Fig.~\ref{fig7}(f)), many quantum algorithms, such as Shor's factorization algorithm \cite{shor1999polynomial} require the error to be as low as $10^{-15}$ \cite{fowler2012surface}. In principle, this low error regime can be reached using quantum error correction protocols to encode information onto the large Hilbert space of many physical qubits, such that error events occurring in a single constituent part can be detected and corrected \cite{terhal2015quantum}. Among these protocols are \textit{stabilizer codes} \cite{gottesman1997stabilizer}, which encode the desired information onto the highly entangled state of many \textit{data qubits}, and perform repeated parity check of predefined groups of data qubits via \textit{ancilla qubits} to avoid collapsing the states of the data qubits. The results can then be decoded to reveal possible errors and provide deterministic correction. This group of data qubits is said to form a \textit{logical qubit}. If the average error probability of physical qubit operations is sufficiently small, the error rate of the logical qubit would be further suppressed if more data qubits are involved. For high physical errors, the logical error becomes worse for larger encoding. The cross-over point is called the \textit{error-threshold} \cite{aharonov2008fault}. As long as the physical error is below the threshold of a certain quantum error correction code, we can scale up the quantum system and implement the correction scheme to reach arbitrarily low logical error rate. The lower the physical error, the fewer number of physical qubits is needed to reach a certain logical error rate. This opens a path toward a fault-tolerant universal quantum computer in the future.

%Also, discuss the surface code after this introduction. Introduce our schematic
The surface code \cite{bravyi1998quantum,dennis2002topological} is a popular stabilizer code due to its relatively high error threshold of about $1\%$ \cite{wang2011surface,fowler2012towards}, and its requirement of only nearest-neighbor coupling, which is suitable for planar architecture. The square lattice topology used to implement the code is depicted in Fig.~\ref{fig0}, with data and ancilla qubits sketched in green and magenta, respectively. They are arranged in a checkerboard pattern, such that each ancilla qubit is coupled to four data qubits. The ancilla qubits are further divided into $X$-syndrome and $Z$-syndrome ones for parity checking of both bit-flip and phase-flip errors. Periodic measurement of a commuting multi-qubit $X$- and $Z$- stabilizers set would project the qubits onto the defined code space. In the rare occasion when an error occurs via the parity check (stabilizers measurement), a decoding protocol is used to update the classical control system to correct for it post-measurement. Thus, error detection, instead of error correction, is the primary focus of surface code implementations \cite{fowler2012surface}. The size of the code is referred to as the \textit{code distance} $d$. A distance-$d$ surface code consists of $d^2$ data qubits and $d^2-1$ ancilla qubits. It can detect $d-1$ errors and correct at most $(d-1)/2$ errors during each parity check cycle. For example, a distance-2 surface code can be implemented using 4 data and 3 ancilla qubits, and is capable of detecting 1 error per cycle, but not correcting it. Upgrading to a distance-3 code would allow detecting up to 2 errors and correcting 1 of them.

\begingroup
\setlength{\tabcolsep}{10pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.5}
\begin{table}[b]
    \caption{\label{tab:pauli_error}Expected average Pauli errors in the processor for different average relaxation times $T_1$.}
        \begin{tabular}{|l||c|c|c|} 
        \hline
          Operation  & \multicolumn{3}{|c|}{Error}   \\
         [0.1ex] 
         \cline{2-4}
          (time) & $300~\mathrm{\mu s}$ &$700~\mathrm{\mu s}$ &$1~\mathrm{m s}$ \\
         \hline\hline
         2Q gate (200 ns) & 5.3e-4& 2.3e-4& 1.6e-4   \\ [0.1ex]
         \hline
         1Q gate (10 ns) & 1.1e-5& 4.7e-6& 3.3e-6 \\[0.1ex]
         \hline
         Readout (200 ns) & 1e-2& 1e-2& 1e-2 \\[0.1ex]
         \hline
         Reset (-) & 1e-2& 1e-2& 1e-2 \\ [0.1ex] 
         \hline
         Idle (2Q) (200 ns) & 2.2e-4& 9.5e-5& 6.6e-5 \\[0.1ex]
         \hline 
         Idle (1Q) (10 ns) & 1.1e-5& 4.7e-6& 3.3e-6 \\[0.1ex]
         \hline 
         Idle (R) (200 ns) & 2.2e-4& 9.5e-5& 6.6e-5 \\[0.1ex]
         \hline 
        \end{tabular}
    \end{table}
    
%Discuss what has been done in superconducting circuits. Optionally, in trapped ions. Mention briefly the bosonic codes.
In superconducting circuits, a distance-2 surface code error detection was implemented on a chip consisting of seven qubits \cite{andersen2020repeated} using a sequential stabilizer-measurement scheme \cite{versluis2017scalable}. This was followed with experimental demonstration of logical operations and the development of process tomography of logical gates, which showed higher performance for fault-tolerant operations compared to non-fault-tolerant ones \cite{marques2021logical}. Along with repetition code, a  distance-2 surface code was also explored using a 53-qubit quantum processor, with the purpose of predicting the performance of larger code sizes \cite{ai2021exponential}. Recently, distance-3 surface code has been implemented \cite{krinner2021realizing,zhao2021realizing}, although lower physical errors will be needed to demonstrate the advantage for higher code distance. A possible major source of error in these works is leakage out of the computational subspace, which is an active research topic \cite{varbanov2020leakage,mcewen2021removing,battistel2021hardware}.

%What we are doing in this section. 
In this section, we estimate the logical errors for large-scale fluxonium processors following surface code error detection and correction scheme. Provided that the physical error is below the threshold, the logical error per round of correction $\epsilon_L$ using a distance-$d$ code follows
\begin{equation}
\label{eqn:logical_error}
    \epsilon_L = C/\Lambda^{(d+1)/2},
\end{equation}
where $C$ is a constant and $\Lambda$ is the suppression factor. In principle, we can simulate $\epsilon_L$ using the estimated error channels, and project the performance of the code to higher distance $d$ based on Eq.~\ref{eqn:logical_error}. For instance, repetition code performance simulation matches well with experimental results when only Pauli error channels are used \cite{ai2021exponential}. Since a majority of the encoding operation consists of Clifford gates, and the surface code stabilizers are Pauli operators, modeling Clifford circuit with Pauli errors is a good approximation.


%Our error budget
We estimate the error budget as follows. The readout and reset error values are taken from state-of-the-art experimental implementation in Ref.~\cite{gusenkova2021quantum}. The measurement time of the qubit with the quantum-limited parametric amplifiers is 200 ns. Since the reset is performed using feedback, and in principle can be done by heralding \cite{johnson2012heralded}, we assume its fidelity is limited by the readout fidelity, and state initialization in the physical qubits can be done instantaneously. We expect the average single-qubit gate time on the chip to be $10$ ns, and two-qubit CZ gate time to be $200$ ns. We note that for small codes, the two-qubit gate time should be at the $\sim 100$ ns range. From these assumption, we can compute the decoherence-limited gate fidelity, given by Eq.~\ref{eqn:decoherence_fidelity}. In addition, we also include errors coming from non-participating (idle) qubits due to decoherence during the operations of participating qubits. We do not take into account non-Markovian noise sources such as leakage and crosstalk, having, on one hand, shown that leakage to higher levels is generally negligible during gate operations, and on the other hand, argued that crosstalk due to spurious coupling is supposed to be suppressed at low frequency. The errors are listed in Table.~\ref{tab:pauli_error} for varying relaxation time $T_1$ of the computational states. All the single- and two-qubit gate errors listed are higher than the average unitary errors simulated in Sections~\ref{sec:single-qubit} and \ref{sec:two_qubit_gates}.

    
\begin{figure}
        \includegraphics[width=0.47\textwidth]{figures/Fig9.pdf}
        \caption{\label{fig10}Logical error for varying surface code distance. We numerically simulate the error for code distance $d=\{3,5,7,9,11\}$, then extrapolate the fit to higher $d$.}
\end{figure}
**Discuss details of numerical simulations. (Shruti + Shraddha)**

**Discuss possible logical operations. (Shruti + Shraddha)**

**Summarize the results. (Long)**

==> sections/9_chipDesign.tex <==
\section{\label{sec:mask}Quantum processor design}

Even when a quantum system shows promising properties in isolated environment, integrating many qubits with well designed control and readout elements in a single device is challenging. In this section, we discuss our design philosophy and simulation framework for a prototypical fluxonium-based quantum information processing device consisting of ten qubits on a planar chip. In addition, we propose approaches to scale up the platform to realize fault-tolerant quantum computing paradigm. We first describe the design of an individual qubit and then a qubit-qubit coupling, before moving on to these more extensive designs.

\subsection{Individual qubits}
First, we discuss individual qubit elements leading to favorable geometry for scaling up. We start with a discussion of a single fluxonium qubit, with coupling to a dual control line and readout resonator, where readout is performed through a bus with a Purcell filter.

The fluxonium qubit is characterized by three energy scales: $E_J$, $E_C$, and $E_L$. While $E_J$ and $E_L$ are determined by the small junction and junction array, respectively, $E_C$ is determined by the capacitive shunt of the qubit's paddles in addition to their coupling to other on-chip components. Thus, it is important to settle on an approximate paddle size and spacing before moving on to lay out the coupling elements to the qubit. With an $E_C \sim 1$ GHz, the capacitive shunt of a fluxonium is relatively small compared to that of a transmon, which translates to the capacitive paddles also being small. In this design, we use floating capacitor paddles as opposed to grounded designs, which may play a role in reducing the sensitivity towards quasiparticle tunneling \cite{kurter2021quasiparticle, vepsalainen2020impact, wilen2021correlated, mcewen2021resolving}. In this architecture, the main parameters of interest are: the $x$ and $y$ dimensions of the paddles, their spacing from each other, and their spacing from the ground plane. A higher capacitance can be achieved from larger paddles, closer spacing between paddles, and closer spacing to the ground plane. Smaller paddle sizes are related to lower quasiparticle tunneling rates \cite{kurter2021quasiparticle}, and they help make the qubit more compact to enable greater scaling. However, the downside of a small paddle size is that it can make appreciable capacitive coupling to the qubit difficult. Here, we settle upon dimensions that yield $E_C \sim 1$ GHz, while balancing the desire for smaller qubit paddles with desirable coupling.

For control, we propose using a dual control line to multiplex DC and RF signals.



As mentioned above, we propose to operate this device using dispersive readout, with the qubit capactively coupled to a readout resonator, which itself is coupled to a bus that acts as a Purcell filter. The readout resonators are $\lambda/4$ resonators, with one open and one closed endpoints. Using $\lambda/4$ instead of $\lambda/2$ resonators, enables us to achieve the same frequency with a shorter length resonator. For a more compact footprint, we inductively couple the readout resonators to the bus, as in their scheme the resonator can terminate next to the bus. Because the qubit frequency is less than $\sim 1$ GHz while the readout resonator frequency is higher at $\sim 7.5$ GHz, the Purcell filter need not be too sharp and has greater tolerance.

\vspace{5 mm}
    
    \emph{Capacitive shunt} [Trevor]
        -The capacitive pad is small. This helps reduce the foot print when scaling up. How do we couple multiple things capacitively to the small pads?
        
        -Normalization of the capacitance by ground plane, which increases the effective capacitance. Classical circuit analysis. Why do we pick this certain geometry/size.
        
        -Floating capacitor pads helps with quasiparticle \cite{kurter2021quasiparticle} as opposed to connected pad design \cite{vepsalainen2020impact,wilen2021correlated,mcewen2021resolving}
        
        
    \emph{Dual control line} [Long & Gerwin] 
        Designing and routing qubit control lines in optimal configurations is an important requirement for scaling up superconducting architectures \cite{krinner2019engineering}. For flux-tunable qubits, reducing the form factor of the chip and hence the microwave resources via multiplexing the flux bias with RF control lines is preferred. This combination of controls is a challenging problem since the requirements on microwave filtering are different for DC and AC couplings.
        
        
        
        
    \emph{Readout bus and resonator} [Trevor & Long]
        -Description of our design. Make the readout resonator smaller. Can fit more qubits
        -No IDC. Coupling similar to Larry's chip. Fit more qubits?
        -Talk about our Purcell bus.
        -Cross-coupling?
        -Multiplexing capabilities \cite{heinsoo2018rapid}

    \emph{Superinductance} [Zahra]
    
\subsection{Multi-qubit coupling} [Trevor, Long, and Brad]

As discussed above, while smaller qubit paddles are advantageous for a smaller footprint, they can introduce difficulties when capacitively coupling the qubit to other circuit elements. In this section, we discuss multi-qubit coupling using a multipath coupler in the context of two qubits, with an extension to a chain more explicitly discussed later. The multipath coupler has two paths: one is a resonator-mediated coupling, while the second is a direct qubit-qubit coupling. 

We target a resonator frequency of $10$ GHz with a qubit-resonator coupling $g = 300$ MHz. While this seems like a relatively high value of $g$ compared to typical transmon designs where larger capacitive paddles are employed, which helps to increase the bare qubit-resonator coupling capacitance, because $g$ scales inversely as the qubit capacitance, the relatively low shunt capacitance of fluxonium makes this desired $g$ value easier to achieve.

We target a direct qubit-qubit coupling of $J_C = 20$ MHz, and we mediate this coupling through a strip of metal with two larger paddles at each end. Modeling this metal strip as only having some capacitance to each qubit paddle and to ground, through a wye-delta transformation, one can see how the capacitance to ground will reduce the effective coupling strength. For a equivalent coupler-qubit capacitances $C_C$ and a coupler capacitance to ground $C_g$, the effective coupling capacitance between qubits is $C_C^2/(2C_C+C_g)$. This significantly constrains the spacing between each qubit, as the capacitance to ground of the direct coupler cannot be too large. Fortunately, this aligns with our goal of reducing the footprint of our coupled qubit design.

\vspace{5 mm}

In general, although the capacitive paddles are small which is nice to reduce the footprint, they can make strong couplings a bit more challenging (though balanced by $C_q$ usually being in the denominator of coupling terms, so that helps)
    
    \emph{Qubit-Resonator coupling} [Trevor & Long]
    
        - What are the requirements?
        - Thought that this might reduce flux crosstalk through ground plane (on the lines of what Gerwin was mentioning in that the control lines on the parametric sample break up the ground plane between flux lines), though not sure at all, and we said we don't really know how to simulate this
        
        Here, we should mention gap, crosstalk is possible, etc.
        
    \emph{Qubit-Qubit coupling} [Trevor]
        Capacitance to ground of the coupling segment reduces the effective qubit-qubit coupling, so need to space the qubits closer together (would also help with smaller footprint)
        
    \emph{Other} ---
        Should we think about effects of cross-capacitance between the coupler elements?

\subsection{Linear chain topology}
    \emph{Sample full mask} ---
        Have some simulations for
        
        Find some references here.
        
\subsection{Square lattice topology}
    \emph{Single plaquette} ---
    
    \emph{Flip-chip} ---
        Proposed design, though won't simulate \cite{rosenberg20173d}

==> sections/a5_chipSim.tex <==
\section{\label{appendix:chipsim}Microwave simulation of quantum processor}
